Computational Diplomacy: How "hackathons for good" feed a participatory future for multilateralism in the digital age

This article explores the role of hackathons for good in building a community of software and hardware developers focused on addressing global SDG challenges. We theorise this movement as computational diplomacy: a decentralised, participatory process for digital governance that leverages collective intelligence to tackle major global issues. Analysing Devpost and GitHub data reveals that 30% of hackathons since 2010 have addressed SDG topics, employing diverse technologies to create innovative solutions. Hackathons serve as crucial kairos moments, sparking innovation bursts that drive both immediate project outcomes and long-term production. We propose that these events harness the neurobiological basis of human cooperation and empathy, fostering a collective sense of purpose and reducing interpersonal prejudice. This bottom-up approach to digital governance integrates software development, human collective intelligence, and collective action, creating a dynamic model for transformative change. By leveraging kairos moments, computational diplomacy promotes a more inclusive and effective model for digital multilateral governance of the future.

==> sections/04_data.tex <==
\section{Data \& Methods}
\label{sec:data}
In order to test the computational diplomacy theory as a form of eco-systemic participatory process largely built through punctual events, we considered {\it hackathons for good} and their long-term activity traces, as exogenous critical shocks, reminiscent of development dynamics in the open source development dynamics \cite{sornette_how_2014}.

Aiming at providing empirical evidence supporting the theory, we studied Devpost \footnote{\url{https://devpost.com}}, the largest hackathon platform, uniting projects held across the globe that are organised in the context of (higher) education, corporations, civic engagement, and others. Most of the events listed are public-facing, meaning that anyone from the general public can register and participate. Participation in hackathons is voluntary, and participants can work on projects that interest them, following the principles of peer-production \cite{benkler_coases_2002}. Most hackathons, however, require projects to be related to a specific theme. These themes can include but are not limited to social good, health, sustainability, and others. The information contained in Devpost is curated by hackathon organisers and participants. 

For this study, we collected data about Devpost hackathons, and their associated projects and participants, between October 2009 and July 2022. For hackathons, we analysed their start dates, the projects submitted to them and the registered participants. Moreover, we considered textual descriptions of hackathons deriving from their themes, tags, and criteria, indicative of the focus and objectives of the event (such as "social good"). Regarding projects, we as well collected the links to the Github repositories in which submission materials --- commonly software code --- were stored. These links were then used to retrieve repository activity statistics (Github Archive, data available for years 2011 to 2022.\footnote{\url{https://gharchives.org}}) For $95,264$ out of $184,652$ projects in our dataset, i.e. $51\%$, a Github repository URL was retrieved and analysed. This allows us to trace software code development before, during and after hackathons for each project. Out of $10,000$ randomly selected repositories, we could retrieve $3,382,144$ event activities in $7,643$ repositories. \footnote{The roughly $25\%$ gap in repositories stems from e.g., private, deleted or migrated repositories, as well as ill-formatted Github URLs}

%\subsection{Data Preprocessing and Quality Control}
Aiming at reconstructing the integrative connections of the Devpost participant-project-hackathon ecosystem, as quality control we excluded projects without an associated hackathon submission ($n=2$,$103$, $1.1\%$ of total retrieved unique project IDs, $n=190,708$) and those submitted to a hackathon for which metadata could not be retrieved ($n=315$, $0.16\%$). In addition, we excluded hackathons for which no project submissions were retrieved ($n=1344$, $19\%$ of total retrieved unique hackathon IDs, $n=7053$). Next, we performed quality control on the participants retrieved, removing those for which project information was not available ($n=242$, $0.07\%$ of total retrieved unique participant IDs, $n=314,430$). To ensure unbiased yearly evolution analysis, we performed an additional quality control involving removing projects launched during years with incomplete tracking. This methodological decision was instrumental for ensuring an unbiased comparison of hackathon and SDG coverage evolution. In this line, we excluded projects in 2009 ($0.04\%$ of all projects, data from October 6, 2009 until the end of year) and in 2022 ($8.8\%$ of all projects, data from January 1, 2022 until July 2, 2022). Note that the timespan of GitHub activity studied for analyzed projects considers 2022 as well since development activity continues after hackathon project completion. After quality control for ensuring a complete hackathon-project-participant linkage and complete year coverage, the dataset for our study contains information about $5,456$ hackathons, which took place between 2009 and 2021 ($5,153$ with complete year resolution), containing all together $184,652$ unique projects ($168,884$ with complete year coverage) and $290,795$ unique participants (undetermined on complete year resolution, not used for analysis).

In order to map SDG alignment of each hackathon in our dataset, we analysed their theme description, the tags associated with each and the text detailing evaluation criteria for adequacy of submitted projects. Using the \textit{text2sdg} R package \cite{meier2022text2sdg}, an API for Large Language Model ensemble SDG word counting, we retrieved all SDG-related words per hackathon theme, tag-set and criteria texts. For preventing double counting, we excluded duplicated SDG words by the combination of SDG, hackathon and text2sdg reference dictionary. To account for the reported SDG specific coverage biases present in the \textit{text2sdg} package \cite{meier2022text2sdg}, we constructed a correction vector to penalise algorithmic decisions as a function of their reported weighted biases. To investigate the relationship between the technologies used in hackathons and their SDG thematic alignment, we applied unsupervised machine learning through hierarchical clustering on a matrix representation of the percentage of times each technology was employed in each SDG hackathon category (technologies were considered for this analysis if they were present in at least 0.1\% of all hackathons analysed). To do so, we calculated Euclidean distances between hackathon technologies with respect to the SDGs tackled and {\it vice versa}. Then, we performed hierarchical clustering using the complete linkage method.


==> sections/appendices/a_SDGs.tex <==
\section{Summary of the 17 UN Sustainable Development Goals (SDGs)}
\label{appendix:SDG}

\begin{enumerate}
    \item \textbf{No Poverty}: Eradicate poverty in all its forms everywhere.
    \item \textbf{Zero Hunger}: End hunger, achieve food security, improve nutrition, and promote sustainable agriculture.
    \item \textbf{Good Health and Well-being}: Ensure healthy lives and promote well-being for all at all ages.
    \item \textbf{Quality Education}: Ensure inclusive and equitable quality education and promote lifelong learning opportunities for all.
    \item \textbf{Gender Equality}: Achieve gender equality and empower all women and girls.
    \item \textbf{Clean Water and Sanitation}: Ensure availability and sustainable management of water and sanitation for all.
    \item \textbf{Affordable and Clean Energy}: Ensure access to affordable, reliable, sustainable, and modern energy for all.
    \item \textbf{Decent Work and Economic Growth}: Promote sustained, inclusive, and sustainable economic growth, full and productive employment, and decent work for all.
    \item \textbf{Industry, Innovation, and Infrastructure}: Build resilient infrastructure, promote inclusive and sustainable industrialisation, and foster innovation.
    \item \textbf{Reduced Inequality}: Reduce inequality within and among countries.
    \item \textbf{Sustainable Cities and Communities}: Make cities and human settlements inclusive, safe, resilient, and sustainable.
    \item \textbf{Responsible Consumption and Production}: Ensure sustainable consumption and production patterns.
    \item \textbf{Climate Action}: Take urgent action to combat climate change and its impacts.
    \item \textbf{Life Below Water}: Conserve and sustainably use the oceans, seas, and marine resources for sustainable development.
    \item \textbf{Life on Land}: Protect, restore, and promote sustainable use of terrestrial ecosystems, manage forests sustainably, combat desertification, and halt biodiversity loss.
    \item \textbf{Peace, Justice, and Strong Institutions}: Promote peaceful and inclusive societies for sustainable development, provide access to justice for all, and build effective, accountable, and inclusive institutions at all levels.
    \item \textbf{Partnerships for the Goals}: Strengthen the means of implementation and revitalise the global partnership for sustainable development.
\end{enumerate}

==> sections/appendices/a_data.tex <==
\section{Data \& Methods}
\label{appendix:data}

\subsection{Devpost}
\label{sec:devpost}
Devpost is an online platform that connects developers with hackathons, coding contests, and challenges, providing a space to showcase projects, collaborate, and gain recognition. It serves as a hub for innovation and skill development, offering opportunities for both novice and experienced developers to engage in competitive programming and project building.

\subsubsection{Key Features}
Devpost hosts and promotes various hackathons and coding contests, both online and in-person, organized by companies, educational institutions, and communities. This allows developers to work on real-world problems and compete for prizes. Developers can create profiles to showcase their projects with detailed descriptions, images, videos, and links to repositories, building a portfolio of their work. The platform facilitates collaboration by enabling users to form teams and connect with industry professionals, mentors, and potential employers.

Participation in Devpost events helps developers learn new technologies, improve coding skills, and gain hands-on experience. Many events include a judging process where industry experts review and provide feedback on projects, helping developers enhance their skills and gain industry insights. Devpost fosters a supportive community where users can share knowledge, ask for help, and support each other, often featuring resources, webinars, and tutorials.

\subsubsection{How Devpost Works}
Users create an account on Devpost to showcase their skills, projects, and event participation. They can browse and register for upcoming hackathons and challenges, each with specific rules, themes, and submission requirements. During events, participants work on their projects individually or in teams and submit them through Devpost, providing all necessary details and documentation.

Projects are then reviewed by judges based on criteria such as creativity, technical complexity, and impact. Winners are announced and awarded prizes, which can include cash, internships, job offers, or other incentives. Submitted projects are showcased on Devpost, allowing other users to view, comment, and share them, leading to networking opportunities and collaboration offers.

\subsubsection{Example Use Cases}
Universities use Devpost to host hackathons that engage students, foster innovation, and provide practical experience outside the classroom. Companies organize coding contests on Devpost to identify talent, crowdsource solutions, and promote their brand within the developer community. Tech communities and non-profit organizations use Devpost to bring developers together to solve social issues and promote learning and collaboration. Individual developers participate in events to challenge themselves, learn new skills, and build a portfolio of projects to showcase to potential employers.

\subsubsection{Benefits of Using Devpost}
Devpost provides exposure and recognition for developers' work, leading to career opportunities. Participation in diverse challenges enhances skills and facilitates networking with like-minded individuals, mentors, and industry professionals. The competitive nature of hackathons and contests inspires innovation and creative problem-solving. Overall, Devpost plays a crucial role in the tech ecosystem by fostering innovation, skill development, and community engagement among developers.

\subsubsection{Limitations of Devpost}

The empirical work presented in this paper is based on an archival analysis of an existing hackathon platform --- Devpost --- and has, as such, several limitations.
First, the database only covers a small number of hackathons that take place across the globe. Moreover, while Devpost contains information about events that take place all over the globe, most events represented there, took place in Europe or the Americas. The data is thus not representative of all hackathons. This does, however, only pose a minor limitation, since we are not aiming for completeness.
Second, the information presented in Devpost is provided by the organisers and participants of events and might, as such, be incomplete or events can be misrepresented. This is a limitation that we have to accept because it is not possible for us to confirm the information that is provided in Devpost. It can, however, be considered unlikely that organisers would greatly misrepresent their event because Devpost is often used to attract participants who would then consequently be disappointed when attending a hackathon that was described very differently.
Third, we make the conceptual assumption that participants attend a hackathon at least partially because of its theme and focus. This is not necessarily the case, though, because individuals might also participate in hackathons for other reasons, such as joining friends who participate. We argue, though, that individuals will still contribute to a hackathon and thus to the SDGs that it focuses on, even if their original motivation might not have been related.
Fourth, due to the way the data was collected, it only represents one specific point in time. Hackathon descriptions and participant profiles might have changed since we collected them. However, since we focus on hackathons that took place in the past, it can be considered unlikely that organisers would change the description of an event post-hoc.
Fifth, it is common for participants to create GitHub repositories specifically for one event and never use them before or after an event. This does not pose an issue for our analysis, though, since it only leads to us potentially underestimating the activity that takes place before and after an event.


\subsection{GitHub Archive}
\label{sec:github_archive}

\subsubsection{GitHub Archive Overview}
GitHub Archive (\url{https://gharchive.org}) is a project that records the public timeline of events on GitHub, offering a comprehensive, continuously updated archive of GitHub activity. It is designed for researchers, developers, and data analysts to analyze trends, behaviors, and patterns in open-source software development.

\subsubsection{General Data Schema}
GitHub Archive captures a variety of event types, and each event follows a specific schema. The general data schema includes:

\begin{enumerate}
    \item {\bf Event Type:} The type of event, such as `PushEvent`, `PullRequestEvent`, `IssuesEvent`, `WatchEvent`, etc.
    \item {\bf Event ID:} A unique identifier for the event.
    \item {\bf Repository:} Details about the repository where the event occurred, including: `id`: Repository ID, `name`: Full name of the repository (`owner/repo`), `url`: URL to the repository.
    \item {\bf Actor:} Information about the user who triggered the event, including: `id`: User ID, `login`: Username, `url`: URL to the user’s GitHub profile.
    \item {\bf Organization (optional):} Information about the organization related to the event, if applicable.
    \item {\bf Payload:} The payload varies depending on the event type and includes detailed information about the event, such as: `PushEvent`: List of commits, commit messages, commit IDs, etc.; `PullRequestEvent`: Pull request details, state, merged status, etc.; For `IssuesEvent`: Issue details, state, comments, etc.
    \item {\bf Public:} A boolean indicating if the event is public.
    \item {\bf Created At:} The timestamp when the event was created.
\end{enumerate}


\subsubsection{Time Ranges and Resolutions}

\begin{itemize}
    \item {\bf Historical Data:} GitHub Archive provides data starting from February 12, 2011.
    \item {\bf Real-time Updates:} Data is continuously updated, capturing real-time GitHub activity.
\end{itemize}

Resolutions: The data is divided into hourly archives. Each hour's data is stored in a JSON file that can be accessed via HTTP or downloaded for local analysis. It can also be downloaded in aggregated monthly or yearly tables.

\subsubsection{Data Accessibility}

\begin{enumerate}
    \item {\bf HTTP Access:} Users can access the hourly JSON files directly via HTTP, enabling them to download specific time periods of data.
    \item {\bf Google BigQuery:} For advanced querying and analysis, the dataset is integrated with Google BigQuery. This allows users to run complex SQL queries on the data without needing to download and store large volumes of JSON files locally.

\end{enumerate}


Example JSON Structure for an Event:
\begin{Verbatim}[breaklines=true]
    {
  "id": "1234567890",
  "type": "PushEvent",
  "actor": {
	"id": 123456,
	"login": "username",
	"display_login": "username",
	"gravatar_id": "",
	"url": "https://api.github.com/ users/
 username",
	"avatar_url": "https:// avatars.githubusercontent.com/ u/123456?"
  },
  "repo": {
	"id": 12345678,
	"name": "owner/repo",
	"url": "https://api.github.com/repos/owner/ repo"
  },
  "payload": {
	"push_id": 1234567890,
	"size": 1,
	"distinct_size": 1,
	"ref": "refs/heads/main",
	"head": "abc123def456",
	"before": "abc123def455",
	"commits": [
  	{
    	"sha": "abc123def456",
    	"author": {
      	"email": "author@example.com",
      	"name": "Author Name"
    	},
    	"message": "Commit message",
    	"distinct": true,
    	"url": "https://api.github.com/repos/ owner/repo/commits/abc123def456"
  	}
	]
  },
  "public": true,
  "created_at": "2024-05-16T12:34:56Z"
}
\end{Verbatim}



GitHub Archive provides a valuable resource for analysing the dynamics of GitHub's open-source ecosystem, offering detailed and structured data for a wide range of applications.

==> sections/appendices/a_summit_of_future.tex <==
\subsection{Multilateralism and The Summit of the Future}
\label{appendix:summit_of_the_future}

\subsubsection{Origins of Multilateralism}
Multilateralism traces its origins to the early twentieth Century, emerging prominently after World War I with the founding of the League of Nations in 1920. This concept was developed to foster international cooperation and prevent conflicts, recognising that many world issues transcend national borders and necessitate collective action. The establishment of the United Nations (UN) after World War II marked a significant advancement in multilateralism, setting a framework for global diplomacy and international law, guided by principles such as sovereign equality and peaceful dispute resolution between nation states.

International organisations under the multilateral framework, such as the United Nations, the World Bank, and the World Health Organisation, aim to address a variety of global issues, including peace and security, economic development, and health crises. Their missions involve promoting human rights, facilitating economic development, mitigating conflicts, and providing humanitarian aid in crises.

However, the efficacy of these organisations is increasingly challenged by a changing world. Current shortcomings include issues like bureaucracy and slow decision-making processes, lack of enforcement mechanisms, disparities in the influence and contribution of member states, and occasionally, a failure to adapt to new global dynamics such as digitisation and climate change. These gaps have sparked debates on the need for reforms to better align with the fast-evolving global landscape, ensuring that multilateralism remains an effective tool for international collaboration in the 21st century.

\subsubsection{The Summit of the Future}
Recognizing the urgency of reforming itself, the United Nations have called to hold the Summit of the Future. This conference, to be held in September 2024, is deemed as a one-of-a-kind moment aiming to redefine and strengthen multilateralism for a better future. Following the recommendations of the High-Level Advisory Board on Effective Multilateralism (HLAB), the Summit of the Future has been designed to reassert the commitments to key international goals such as the Sustainable Development Goals (SDGs), the UN Charter, and to promote a rejuvenated, more effective multilateral system that can positively impact people's lives worldwide. The backdrop to this summit includes recent global crises such as the climate emergency, the COVID-19 pandemic, the war in Ukraine, and exponentially paced technological changes disrupting the socioeconomic landscape. These extreme events along with many, however not less disruptive, local events, have tested the resilience and efficacy of international institutions, which have been primarily designed to support multilateralism and to alleviate human and social disasters. Emphasising the urgent need for unified action based on shared principles and objectives, UN Secretary-General António Guterres highlighted the summit as a unique chance to rebuild trust and align outdated multilateral frameworks with today's global landscape, characterised by equity and solidarity. It aims to mitigate risks and foster a safer, more peaceful world. The Summit of the Future is organised around 6 shifts: 
Rebuild Trust in Multilateralism: Improve legitimacy and effectiveness through inclusion and accountability
Planet and People: Regain balance with nature and provide clean energy for all
Global Finance: Ensure sustainable finance that delivers for all	
Digital and Data Governance: Support a just digital transition that unlocks the value of data and protects against digital harms							
Peace and Prevention: Empower effective, equitable collective security arrangements
Anticipatory Action: Strengthen governance for current and emerging transnational risks




At its core, the Summit of the Future is driven by the vision laid out in the Secretary-General's 2021 report, ``Our Common Agenda," which advocates for an inclusive, networked, and efficient form of multilateralism. This initiative seeks to accelerate progress towards the 17 SDGs, with a concerted effort to overcome setbacks caused by the pandemic and other global challenges. A key outcome expected from the summit is the adoption of the Pact for the Future, encompassing five critical areas: sustainable development and financing, international peace and security, science, technology, innovation and digital cooperation, youth and future generations, and transforming global governance. This pact is seen as a commitment among nations to leverage global tools to address emergent issues proactively .
One of the six shifts emphasized in the preparatory discussions for the Summit involves new forms of people engagement and collective intelligence, crucial for rebuilding trust in multilateralism. This shift acknowledges the imperative of involving a broader spectrum of society in decision-making processes, particularly the youth. With over half of the world's population under 30, the summit emphasizes the need for young people to have a meaningful seat at the decision-making table. This approach is not just about consulting young people but involves recognizing them as true and equal partners in crafting a sustainable future.
The discussions and policy briefs leading up to the Summit have underscored the need for a more networked, inclusive, and effective UN system to accelerate SDG implementation. This entails fostering enablers of SDG acceleration, such as digitalization and access to finance, addressing obstacles to SDG realization, reinforcing international standards supportive of SDGs, and enhancing UN development cooperation and financing. The overarching goal is to bridge the significant gap between global challenges and the UN's capacity to respond effectively, thereby strengthening international cooperation and trust, especially among developing nations.
In essence, the Summit of the Future aims to catalyze a global movement towards more effective, inclusive, and networked multilateralism. By embracing new forms of engagement and leveraging collective intelligence, the summit seeks to establish a more resilient, equitable, and sustainable framework for addressing the complex challenges of today and tomorrow.

